Do You Think You Can Hold Me? The Real Challenge of Problem-Space Evasion Attacks

Android malware is a spreading disease in the virtual world. Anti-virus and detection systems continuously undergo patches and updates to defend against these threats. Most of the latest approaches in malware detection use Machine Learning (ML). Against the robustifying effort of detection systems, raise the \emph{evasion attacks}, where an adversary changes its targeted samples so that they are misclassified as benign. This paper considers two kinds of evasion attacks: feature-space and problem-space. \emph{Feature-space} attacks consider an adversary who manipulates ML features to evade the correct classification while minimizing or constraining the total manipulations. \textit{Problem-space} attacks refer to evasion attacks that change the actual sample. Specifically, this paper analyzes the gap between these two types in the Android malware domain. The gap between the two types of evasion attacks is examined via the retraining process of classifiers using each one of the evasion attack types. The experiments show that the gap between these two types of retrained classifiers is dramatic and may increase to 96\%. Retrained classifiers of feature-space evasion attacks have been found to be either less effective or completely ineffective against problem-space evasion attacks. Additionally, exploration of different problem-space evasion attacks shows that retraining of one problem-space evasion attack may be effective against other problem-space evasion attacks.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> idconserved.tex <==
\section{Identifying Conserved Features}
\label{sec:CF}

%Having demonstrated the effectiveness of conserved features in bridging the gap between realizable and feature space evasion models, 
We now describe a systematic automated procedure for identifying these. 
%\textcolor{red}{
We first introduce how to identify conserved features of SL2013, and then describe how to generalize the approach to extract conserved features of Hidost.
%present how these features are further employed to identify conserved features of other classifiers.  
%}

The key to identifying the conserved features of a malicious PDF is to discriminate them from non-conserved ones.
Since merely applying statistical approaches on training data is insufficient to discriminate between these two classes of features, as demonstrated above, we need a qualitatively different approach which relies on the nature of evasions (as implemented in EvadeML) and the sandbox (which determines whether malicious functionality is preserved) to identify features that are conserved.
%Instead, we use a systematic approach to identify conserved features. 

We use a modified version of pdfrw \cite{pdfrw}\footnote{The modified version is available at \url{https://github.com/mzweilin/pdfrw}.} to parse the objects of PDF file 
%with a logic structure as shown on the right-hand side of Figure \ref{pdf-structure} 
and repack them to produce a new PDF file. We use Cuckoo \cite{Guarnieri} as the sandbox to evaluate malicious functionality. 
In the discussion below, we define $x_i$ to be the malicious file, $\mathsf{S}_i$ the conserved feature set of $x_i$, and $\mathsf{O}_i$ the set of its non-conserved features. 
Initially, $\mathsf{S}_i = \mathsf{O}_i = \emptyset$.

At the high level, our first step is to sequentially delete each object of a malicious file and eliminate non-conserved features by evaluating the existence of a malware signature in a sandbox for each resulting PDF, which provides a preliminary set of conserved features. Then, we replace the object of each corresponding structural path in the resulting preliminary set with an external benign object and assess the corresponding functionality, which allows us to further prune non-conserved features. 
Next, we describe these procedures in detail.

\subsection{Structural Path Deletion}

In the first step, we filter out non-conserved features by deleting each object and its corresponding structural path, and then checking whether this eliminates malicious functionality (and should therefore be conserved). First, we obtain all the structural paths (objects) by parsing a PDF file. These objects are organized as a tree-topology and are sequentially deleted. Each time an object is removed, we produce a resulting PDF file by repacking the remaining objects. Then, we employ the sandbox to detect malicious functionality of the PDF after the object deletion. If any malware signature is captured, the corresponding structural path of the object is deleted as a non-conserved feature, and added to $\mathsf{O}_i$. On the other hand, if no malware signature is detected, the corresponding feature is added in $\mathsf{S}_i$ as a \emph{possibly} conserved feature.

One important challenge in this process is that features are not necessarily independent.
Thus, in addition to identifying $\mathsf{S}_i$ and $\mathsf{O}_i$, we explore \emph{interdependence} between features by deleting objects. 
As the logic structure of a PDF file is with a tree-topology, the presence of some structural path depends on the presence of other structural paths whose object refers to the object of the prior one. 
%For example in some PDFs, the presence of \verb|/OpenAction/JS| and \verb|/OpenAction/S| depend on \verb|/OpenAction|. If the object \verb|OpenAction| is deleted, so as its structural path \verb|/OpenAction|, then both \verb|/OpenAction/JS| and \verb|/OpenAction/S| are deleted as well. We call \verb|/OpenAction/JS| and \verb|/OpenAction/S| as the dependents of \verb|/OpenAction|. 
We define that a structural path is a dependent of another if unilateral deleting the object associated with the latter causes a flip from 1 to 0 on the feature value of the former.
For any feature $j$ of $x_i$, we denote the set of features that depend on $j$ by $\mathsf{D}_i^{j}$.
Note that for a given structural path (feature), there could be multiple corresponding PDF objects. In such a case, these objects are deleted simultaneously, so as the corresponding feature value is shifted from 1 to 0. 

\subsection{Structural Path Replacement}

In the second step, we subtract the remaining non-conserved features in the preliminary $\mathsf{S}_i$ and move them to $\mathsf{O}_i$. Similar to the prior step, we first obtain all the structural paths and objects of the malicious PDF file. Then for each object of the PDF that is in $\mathsf{S}_i$, we replace it with an external object from a benign PDF file and produce the resulting PDF, which is further evaluated in the sandbox. If the sandbox detects any malware signature, then the corresponding structural path of the object replaced is moved from $\mathsf{S}_i$ to $\mathsf{O}_i$. Otherwise, the structural path is a conserved feature since both deletion and replacement of the corresponding object removes the malicious functionality of the PDF file. Note that in the case of multiple corresponding and identical objects of a structural path, all of these objects are replaced simultaneously.


After structural path deletion and replacement, for each malicious PDF file $x_i$, we can get its conserved feature set $\mathsf{S}_i$, non-conserved feature set $\mathsf{O}_i$, and dependent feature set $\mathsf{D}_j$ for any feature $j \in \mathsf{S}_i  \cup \mathsf{O}_i$, which could be further leveraged to design evasion-robust classifiers.  

\subsection{Obtaining a Uniform Conserved Feature Set}

The systematic approach discussed above provides a conserved feature set for each malicious seed to retrain a classifier. 
Our goal, however, is to identify a single set of conserved features which is \emph{independent} of the specific malicious PDF seed file.
We now develop an approach for transforming a collection of $\mathsf{S}_i$, $\mathsf{O}_i$, and $\mathsf{D}_i^{j}$ for a set of malicious seeds $i$ into a \emph{uniform} set of conserved features.

\renewcommand{\algorithmicrequire}{ \textbf{Input:}} %Use Input in the format of Algorithm  
\renewcommand{\algorithmicensure}{ \textbf{Output:}} %UseOutput in the format of Algorithm 



Obtaining a uniform set of conserved features faces two challenges: 1) minimizing conflicts among different conserved features, as a conserved feature for one malicious instance could be a non-conserved feature for another, and 2) abiding by feature interdependence if a conserved feature should be further eliminated. 

\begin{algorithm}     
\begin{algorithmic}[1]  
\REQUIRE ~~\\
The set of conserved features for $x_i(i \in [1,n])$, $\mathsf{S}_i$;\\  
The set of non-conserved features for $x_i(i \in [1,n])$, $\mathsf{O}_i$;\\
The set of dependent features for $j \in \mathsf{S}_i \cup \mathsf{O}_i$ , $\mathsf{D}_i^j$; 
\ENSURE ~~\\   
The uniform conserved feature set for $\{x_1,x_2,...,x_n\}$, $\mathsf{S}$;
\STATE $\mathsf{S} \leftarrow \bigcup_{i=1}^n \mathsf{S}_i$;
\STATE $\mathsf{S}^{'} \leftarrow \mathsf{S}$;
\STATE $\mathsf{Q} \leftarrow \emptyset$;
\STATE $\mathsf{D}^j = \bigcup_{i=1}^n \mathsf{D}_i^j$;
\FOR{each $j \in \mathsf{S}^{'}$}
\IF{$j \notin \mathsf{Q}$}
\IF{$\sum_{i=1}^n \mathbbm{1}_{j \in \mathsf{O}_i} \geq \beta\cdot\sum_{i=1}^n \mathbbm{1}_{j \in \mathsf{S}_i}$}
\STATE $\mathsf{S} \leftarrow \mathsf{S} \setminus (\{j\} \cup \mathsf{D}^j)$;
\STATE $\mathsf{Q} \leftarrow \mathsf{Q} \cup (\{j\} \cup \mathsf{D}^{j})$;
\ENDIF
\ENDIF  
\ENDFOR  
\RETURN $\mathsf{S}$;  
\end{algorithmic}
\caption{ Forward Elimination for uniform conserved feature set.}
%\vspace{-0.15in}   
\label{alg:uniform} 
\end{algorithm}

To address these challenges,  we propose a \emph{Forward Elimination} algorithm to compute the uniform conserved feature set for a set of malicious seeds $\{x_1,x_2,...,x_n\}$, given the conserved feature sets, non-conserved feature sets and dependent sets for each seed. 
As Algorithm \ref{alg:uniform} shows, we first obtain a union of the conserved feature sets. Then, we explore the contradiction of each feature in the union with the others, by comparing the total number of the feature being selected as a non-conserved feature and conserved feature. If the former one is greater than $\beta$ times the latter one, then this feature, together with its dependents, are eliminated from the union. Otherwise, the feature is added to the uniform feature set. We use $\beta$ as a parameter to adjust the balance between conserved and non-conserved features. Typically, $\beta > 1$  as we are inclined to preserve malicious functionality associated with a conserved feature, even it could be a non-conserved feature of another PDF file. We set $\beta = 3$ in our experiments.

\subsection{Identifying Conserved Features for Other Classifiers}

Once we obtain conserved features of SL2013 for each malicious seeds, we can employ these features to identify conserved features for other classifiers using binary features. 
As our approach relies on the existence of malicious functionality and corresponding features, such a relation is not obvious for real-valued features; we therefore leave the question of how to define and identify conserved features in real space for future work.

\noindent{\bf Hidost} Hidost and SL2013 are similar in nature in such a way that they employ structural paths as features. 
The only difference is that Hidost consolidates features of SL2013 as described in Section~\ref{S:exp}.
Therefore, once the conserved features of SL2013 are identified, we can simply apply the \emph{PDF structural path consolidation rules} described in Srndic and Laskov~\cite{srndic2016} to transform these features to the corresponding conserved features for Hidost.

\noindent{\bf Binarized PDFRate} We identify the conserved features for PDFRate-B by using the conserved feature set $\mathsf{S}_i$ of each seed $x_i$. 
For each $x_i$, we generate $|\mathsf{S}_i|$ PDF files, each of which corresponds to the PDF file when an element (structural path) in $\mathsf{S}_i$ is deleted.
We then compare PDFRate-B features of these PDFs to the original $x_i$. 
If any feature value of $x_i$ is flipped from 1 to 0, then this feature will be added in the conserved feature set of $x_i$ for PDFRate-B.
Afterward, we use Algorithm \ref{alg:uniform} to obtain the uniform conserved feature set.
This approach can in fact be used for arbitrary PDF malware detectors over binary features (leveraging conserved structural paths identified using SL2013).

\subsection{Conserved Features}
\label{appendix:cf}
%In our experiments, we identified a subset of the features as the conserved feature set for the classifiers in our case study; see 
Table~\ref{table:cf} presents the full list of conserved features we identified for each classifier.
%\begin{itemize}%[noitemsep]
%
%\item \textbf{SL2013}:
%	\begin{flushleft}
%	\verb|/Names| \\
%	\verb|/Names/JavaScript| \\
%	\verb|/Names/JavaScript/Names| \\
%	\verb|/Names/JavaScript/JS| \\
%	\verb|/OpenAction| \\
%	\verb|/OpenAction/JS| \\
%	\verb|/OpenAction/S| \\
%	\verb|/Pages| \\
%	\end{flushleft}
%
%\item \textbf{Hidost}:
%	\begin{flushleft}
%	\verb|/Names| \\
%	\verb|/Names/JavaScript| \\
%	\verb|/Names/JavaScript/Names| \\
%	\verb|/Names/JavaScript/JS| \\
%	\verb|/OpenAction/JS| \\
%	\verb|/OpenAction/S| \\
%	\verb|/Pages| \\
%	\end{flushleft}
%
%\item \textbf{PDFRate-B}:
%	\begin{flushleft}
%	\verb|count_box_other| \\
%	\verb|count_javascript| \\
%	\verb|count_js| \\
%	\verb|count_page| \\
%	\end{flushleft}
%\end{itemize}

\begin{table}[t]
\centering
\scalebox{0.8}{

\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Classifier}                 & \textbf{Conserved features}         & \multicolumn{3}{c|}{Involve JS?} \\ \hline\hline
\multirow{8}{*}{SL2013}    & /Names                     & \multicolumn{3}{c|}{No}                     \\ \cline{2-5} 
                           & /Names/JavaScript          & \multicolumn{3}{c|}{Yes}                    \\ \cline{2-5} 
                           & /Names/JavaScript/Names    & \multicolumn{3}{c|}{Yes}                    \\ \cline{2-5} 
                           & /Names/JavaScript/Names/JS & \multicolumn{3}{c|}{Yes}                    \\ \cline{2-5} 
                           & /OpenAction                & \multicolumn{3}{c|}{No}                     \\ \cline{2-5} 
                           & /OpenAction/JS             & \multicolumn{3}{c|}{Yes}                    \\ \cline{2-5} 
                           & /OpenAction/S              & \multicolumn{3}{c|}{No}                     \\ \cline{2-5} 
                           & /Pages                     & \multicolumn{3}{c|}{No}                     \\ \hline \hline
\multirow{7}{*}{Hidost}    & /Names                     & \multicolumn{3}{c|}{No}                     \\ \cline{2-5} 
                           & /Names/JavaScript          & \multicolumn{3}{c|}{Yes}                    \\ \cline{2-5} 
                           & /Names/JavaScript/Names    & \multicolumn{3}{c|}{Yes}                    \\ \cline{2-5} 
                           & /Names/JavaScript/Names/JS & \multicolumn{3}{c|}{Yes}                    \\ \cline{2-5} 
                           & /OpenAction                & \multicolumn{3}{c|}{No}                     \\ \cline{2-5} 
                           & /OpenAction/JS             & \multicolumn{3}{c|}{Yes}                    \\ \cline{2-5} 
                           & /Pages                     & \multicolumn{3}{c|}{No}                     \\ \hline \hline
\multirow{4}{*}{PDFRate-B} & count\_box\_other          & \multicolumn{3}{c|}{No}                     \\ \cline{2-5} 
                           & count\_javascript          & \multicolumn{3}{c|}{Yes}                    \\ \cline{2-5} 
                           & count\_js                  & \multicolumn{3}{c|}{Yes}                    \\ \cline{2-5} 
                           & count\_page                & \multicolumn{3}{c|}{No}                     \\ \hline 
\end{tabular}

}

\caption{Conserved features and  their relevance to JavaScript.}
\label{table:cf}
\end{table}

\subsection{Conserved vs. Regularized Features}
\label{appendix:regularized-features}
In our experiments, we empirically adjust the SVM parameter $C$ to study the overlap between \emph{conserved features} and those selected by $l_1$ regularization. 
We first adjust $C$ to perform feature reduction until the number of features is identical to the number of conserved features.
In this case, sparse versions of both SL2013 and Hidost include only 3 of the conserved features, while sparse PDFRate-B includes only 1.
In another experiment, we adjusted $C$ until all conserved features were selected.
In this case, SL2013 requires 510 features, Hidost needs 154, and PDFRate-B needs 83.
%We then adjust $C$ until the features selected by regularization contain all the conserved features.
%The results are summarized in Table~\ref{table:cf-regu}.

%\begin{table}[t]
%\centering
%\begin{tabular}{|c|c|c|}
%\hline
%Classifiers                & \# Features & \# Overlaps with CF \\ \hline \hline
%\multirow{2}{*}{SL2013}    & 8           & 3                                   \\ \cline{2-3} 
%                           & 510         & 8                                   \\ \hline
%\multirow{2}{*}{Hidost}    & 7           & 3                                   \\ \cline{2-3} 
%                           & 154         & 7                                   \\ \hline
%\multirow{2}{*}{PDFRate-B} & 4           & 1                                   \\ \cline{2-3} 
 %                          & 83          & 4                                   \\ \hline
%\end{tabular}
%\caption{Conserved vs. regularized features}
%\label{table:cf-regu}
%\end{table}
